Once Upon a $\textit{Time}$ in $\textit{Graph}$: Relative-Time Pretraining for Complex Temporal Reasoning

Our physical world is constantly evolving over time, rendering challenges for pre-trained language models to understand and reason over the temporal contexts of texts. Existing work focuses on strengthening the direct association between a piece of text and its time-stamp. However, the knowledge-time association is usually insufficient for the downstream tasks that require reasoning over temporal dependencies between knowledge. In this work, we make use of the underlying nature of time, all temporally-scoped sentences are strung together through a one-dimensional time axis, and suggest creating a graph structure based on the relative placements of events along the time axis. Inspired by the graph view, we propose RemeMo ($\underline{Re}$lative Ti$\underline{me}$ $\underline{Mo}$deling), which explicitly connects all temporally-scoped facts by modeling the time relations between any two sentences. Experimental results show that RemeMo outperforms the baseline T5 on multiple temporal question answering datasets under various settings. Further analysis suggests that RemeMo is especially good at modeling long-range complex temporal dependencies. We release our code and pre-trained checkpoints at $\href{https://github.com/DAMO-NLP-SG/RemeMo}{\text{this url}}$.

==> sections/analysis.tex <==
\section{Analysis}

==> tables/exp-ablation-trc.tex <==
\begin{table}[!t]
    \centering
    % \small
    \resizebox{1.0\columnwidth}{!}{
    % \begin{tabular}{l|cc|cc|cc|cc|cc|cc|cc|cc|cc}
    \begin{tabular}{lcccccccc}
    \specialrule{.12em}{1em}{0em}
    % \specialrule{.1em}{.05em}{.05em}
    % \hline
         & \multicolumn{4}{c}{\textbf{TimeQA}} & \multicolumn{2}{c}{\textbf{TempReason}} & \multicolumn{2}{c}{\multirow{2}{*}{\textbf{SituatedQA}}} \\
         % \cline{1-14}
        % \cdashline{1-13}[2pt/3pt]
         & \multicolumn{2}{c}{\textbf{Easy}} & \multicolumn{2}{c}{\textbf{Hard}} & \multicolumn{2}{c}{\textbf{ReasonQA L3}} & &  \\
          & F1 & EM & F1 & EM & F1 & EM & F1 & EM \\
         \hline
        \textsc{RemeMo}$_{\text{\texttt{base}}}$ & 70.35 & 61.36 & 67.28 & 58.19 & 91.17 & 89.29 & 55.06 & 48.12 \\
        No TRC                                   & 69.81 & 61.06 & 65.71 & 56.99 & 62.71 & 53.91 & 54.07 & 47.19 \\
    % \specialrule{.05em}{1em}{0em}
    \specialrule{.12em}{.05em}{.0em}
    % \hline
    \end{tabular}
    }
    % \vspace{5pt}
    \caption{Ablation results about the Time Relation Prediction (TRC) objective in LM pre-training. These results are under the single-context setting. }
    \label{tab:exp:ablation:trc}
\end{table}


